VGI-Bench: Probing Visual Intelligence in Video Generation Models

Recent studies suggest that video generation models can exhibit certain forms of zero-shot visual reasoning through generated frames. Yet reliable evaluation remains challenging: benchmarks should adopt inputs aligned with the visual priors of current video models, require valid evolving processes rather than only plausible final states, and calibrate task difficulty to remain challenging yet partly feasible. To this end, we introduce VGI-bench, containing 27 tasks and 810 instances, organized by a two-level taxonomy of task domains and skill tags for fine-grained evaluation of visual reasoning capabilities of video generation models. Our evaluations show that current generative systems can solve a subset of visually grounded reasoning tasks, but remain far from reliable, with even the strongest model, Seedance 2.0, achieving only 51.0% under our evaluation criteria. Our analysis further explore the output failure modes, input condition sensitivity, performance transfer boundary from synthetic fine-tuning, and internal denoising perspective revealing limited self-correction, where later steps mainly refine early hypotheses rather than correct reasoning errors. We hope VGI-bench will help stimulate the development of next-generation video generation models. Website: https://hexuan21.github.io/VGI-Bench/

==> Tables/4_subset_video_input_res.tex <==
\begin{table}[t]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.1}
\resizebox{\columnwidth}{!}{%
\newcolumntype{G}{>{\columncolor{gray!8}[2pt][2pt]}c}
\begin{tabular}{l c@{\hskip 3pt}G c@{\hskip 3pt}G c@{\hskip 3pt}G c@{\hskip 3pt}G c@{\hskip 3pt}G}
\toprule
 & \multicolumn{2}{c}{\textbf{Sora2}} & \multicolumn{2}{c}{\textbf{Veo3.1}} & \multicolumn{2}{c}{\textbf{Kling3.0}} & \multicolumn{2}{c}{\textbf{Sdce2.0}} & \multicolumn{2}{c}{\textbf{Wan2.7}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
 & Comp. & Rub. & Comp. & Rub. & Comp. & Rub. & Comp. & Rub. & Comp. & Rub. \\
\arrayrulecolor{gray!50}\midrule\midrule\arrayrulecolor{black}
Easy    & & & & & & & & & & \\
Mid     & & & & & & & & & & \\
Hard    & & & & & & & & & & \\
\arrayrulecolor{gray!50}\midrule\arrayrulecolor{black}
Overall & & & & & & & & & & \\
\bottomrule
\end{tabular}%
}
\caption{Evaluation results on the video-input subset of our benchmark. Only models that support video extension as input (\textit{Sora2}, \textit{Veo3.1}, \textit{Kling3.0}, \textit{Sdce2.0}, \textit{Wan2.7}) are evaluated. Scoring follows the same Completeness (Comp.) and Checklist Score (Rub.) protocol as Table~\ref{tab:main_res}; higher is better.}
\label{tab:subset_video_input_res}
\end{table}


==> Tables/apdx_vbvr_sft_per_domain.tex <==
% 3-lv canonical view (build_release stripe), TASK_LEVEL_EXCLUDE/TASK_EXCLUDE honored.
% Combined table: per-domain (top) + per-skill (bottom, via \input), one shared caption.
\begin{table}[ht]
\centering
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c c}
\toprule
\textbf{Model}
 & \makecell{Structured\\Puzzles}
 & \makecell{Visual\\Organization}
 & \makecell{Spatiotemporal\\Dynamics}
 & \makecell{Physical\\Manipulation}
 & \textbf{Overall} \\
\midrule
\texttt{Wan2.2-I2V}  & 11.6 & 21.4 & 30.2 & 24.4 & 21.5 \\
\texttt{VBVR-Wan2.2} & \cellcolor{hlgreen!42}53.2\,{\footnotesize\textcolor{Green}{$\uparrow$41.6}}
                     & \cellcolor{hlgreen!16}37.6\,{\footnotesize\textcolor{Green}{$\uparrow$16.2}}
                     & \cellcolor{hlred!5}29.0\,{\footnotesize\textcolor{Red}{$\downarrow$1.2}}
                     & \cellcolor{hlgreen!18}42.6\,{\footnotesize\textcolor{Green}{$\uparrow$18.1}}
                     & \cellcolor{hlgreen!20}41.2\,{\footnotesize\textcolor{Green}{$\uparrow$19.7}} \\
\bottomrule
\end{tabular}%
}
\\[0.9em]
\input{Tables/apdx_vbvr_sft_per_skill}
\vspace{-0.4em}
\caption{Per-domain (top) and per-skill (bottom) performance (final score) breakdown for \texttt{VBVR-Wan2.2} vs.\ base \texttt{Wan2.2-I2V}.}
\label{tab:apdx_vbvr_sft_skill}
\label{tab:apdx_vbvr_sft_domain}
\end{table}


==> Tables/apdx_vbvr_sft_per_skill.tex <==
% Per-skill tabular fragment; included by Tables/5_vbvr_sft_per_domain.tex
% (the combined per-domain + per-skill table), which owns the table env,
% caption, and labels.
% inline skill-icon helper: glyph + bold name
\providecommand{\skicon}[2]{%
  \raisebox{-0.2em}{\includegraphics[height=1.1em]{Figures/skill_icons/skill_#1.png}}\,\textbf{#2}%
}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l c c c c}
\toprule
\textbf{Model}
 & \skicon{planning}{Planning}
 & \skicon{spatial}{Spatial}
 & \skicon{temporal}{Temporal}
 & \skicon{attribute_grounding}{\makecell{Attribute\\Grounding}} \\
\midrule
\texttt{Wan2.2-I2V}  & 10.4 & 26.4 & 37.0 & 17.8 \\
\texttt{VBVR-Wan2.2} & \cellcolor{hlgreen!34}44.1\,{\footnotesize\textcolor{Green}{$\uparrow$33.7}}
                     & \cellcolor{hlgreen!11}37.3\,{\footnotesize\textcolor{Green}{$\uparrow$10.9}}
                     & \cellcolor{hlred!11}25.8\,{\footnotesize\textcolor{Red}{$\downarrow$11.2}}
                     & \cellcolor{hlgreen!20}37.9\,{\footnotesize\textcolor{Green}{$\uparrow$20.1}} \\
\midrule
\textbf{Model}
 & \skicon{spring}{Physics}
 & \skicon{affordance}{Affordance}
 & \skicon{topology}{Topology}
 & \\
\midrule
\texttt{Wan2.2-I2V}  & 27.6 & 43.7 &  5.4 & \\
\texttt{VBVR-Wan2.2} & \cellcolor{hlgreen!12}39.9\,{\footnotesize\textcolor{Green}{$\uparrow$12.3}}
                     & \cellcolor{hlgreen!12}55.2\,{\footnotesize\textcolor{Green}{$\uparrow$11.5}}
                     & \cellcolor{hlgreen!21}26.3\,{\footnotesize\textcolor{Green}{$\uparrow$20.9}}
                     & \\
\bottomrule
\end{tabular}%
}

